Promoting Fair Proposers, Fair Responders or Both? Cost-Efficient Interference in the Spatial Ultimatum Game

Institutions and investors face the constant challenge of making accurate decisions and predictions regarding how best they should distribute their endowments. The problem of achieving an optimal outcome at minimal cost has been extensively studied and resolved using several heuristics. However, these works usually fail to address how an external party can target different types of fair behaviour or do not take into account how limited information can shape this complex interplay. Here, we consider the well-known Ultimatum game in a spatial setting and propose a hierarchy of interference mechanisms based on the amount of information available to an external decision-maker and desired standards of fairness. Our analysis reveals that monitoring the population at a macroscopic level requires more strict information gathering in order to obtain an optimal outcome and that local observations can mediate this requirement. Moreover, we identify the conditions which must be met for an individual to be eligible for investment in order to avoid unnecessary spending. We further explore the effects of varying mutation or behavioural exploration rates on the choice of investment strategy and total accumulated costs to the investor. Overall, our analysis provides new insights about efficient heuristics for cost-efficient promotion of fairness in societies. Finally, we discuss the differences between our findings and previous work done on the PD and present our suggestions for promoting fairness as an external decision-maker.

==> IJCAI/Introduction.tex <==
% !TEX root = ijcai18.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}
\label{section:intro}
The problem of understanding and predicting  collective behaviours of agents in evolving multiagent systems is a well studied research topic in evolutionary game theory, as it can be found in a variety of real-world situations, ranging from ecosystems to human organisations and social networks~\cite{santos2006pnas,Sigmund2001PNAS,tuyls2007evolutionary,RaghunandanS12,HanJaamas2016,SahraeiBBTW14}. In this context, cooperation is typically assumed to emerge from the combined actions of participating agents within the system. 
%For example, in a country's political scene, cooperative behaviour is encouraged by its participating political parties, in order to achieve economical prosperity. 
%Similarly, in wildlife ecosystems, cooperation is assumed to be advocated by the members of the species in order to survive.
%
However, in many scenarios, such behaviours are advocated and promoted by an \emph{exogenous agent}, which  is not part of the system, calling for a new set of heuristics capable of {\it engineering} a desired collective behaviour in a self-organised multiagent system. 
%For example, consider an international political/economical organisation (e.g., the United Nations, or the European Union) that is not part of a certain country's political life (and thus, can be considered as an outsider from that country's political parties' perspective), decides to promote a certain preferred political behaviour. 
%To do so, the organisation can provide financial support to political parties that choose to follow the preferred politics. 
%However, for the organisation, this political investment comes with a (financial) cost in the form of monetary expenses. 
%Thus, from a decision-maker perspective, a key challenge for the organisation is to decide whether and how to \emph{interfere} (i.e., invest to achieve certain changes) in that country's political scene, such that the desired political situation is achieved, while the total cost of interference (i.e., investment cost) is minimised.
%
For instance, consider a wildlife management organisation (e.g., the WWF) that aims  to maintain a desired level of biodiversity in a particular region.
To do so, the organisation,  not being  part of the region's eco-system, has to decide whether to modify the current population of some species, and if so, then when, and in what degree to \emph{interfere} in the eco-system (i.e., to modify the composition and the biodiversity of the population)~\cite{levin2000multiple}.
Note that since more efficient population controlling typically implies more physical actions, which requires higher (monetary) expenses in both human resources and equipment, the organisation has to achieve a balance between efficient wildlife management and a low total investment cost. 
Moreover, due to the evolutionary dynamics of the eco-system (e.g., frequency and structure dependence \cite{santos2006pnas}), undesired behaviours can reoccur over time, for example when the interference was not sufficiently strong in the past. 
Given this, the decision-maker also has to take into account the fact that she will have to repeatedly interfere in the eco-system in order to sustain the level of biodiversity over time.
That is, she has to find an efficient sequential interference strategy that leads to her desired goals, while also minimising the total cost of interference.

Although the (sequential) decision-making literature provides a number of techniques to tackle similar problems where the goal is to provide a sequence of decisions that lead to optimal behaviour of the system (e.g., the desired level of biodiversity) while minimising the total cost of making such decisions~\cite{Madani2004,GuhaMunagala2007,Bachrach2009,Tran-Thanh2012,DingEtAl2013}, these approaches typically ignore the fact that the agents, with whom the decision-maker has to interact, also have their own strategic behaviours that together drive the (evolutionary) dynamics of the system. 
Given this, we argue that such solutions will not be able to exploit the system characteristics, and thus, will fail in providing efficient performance in achieving the desired system status (e.g., the status quo between the fighting opponents, or the desired diversity of population).
%
On the other hand, game theoretic literature, which deals with these strategic behaviours, typically focuses on the extremes of the problem. 
In particular, researchers either assume that the system is fully closed (i.e., there are no outsider decision-makers) or the decision-maker has full control over the behaviour of the agents.
Typical models for the former are classical (both non-cooperative and coalitional) game theoretical models~\cite{Bachrach2009,AzizBH10,AadithyaMJ11}. 
The latter includes models from mechanism design, where the decision-maker is the system designer, and can define some set of norms and penalties such that the agents are  incentivised not to deviate from the desired behaviour~\cite{endriss2011incentive,Wooldridge12,LevitEtAl2013,HarrensteinTW14}. 
Given this, these works are not suitable to meet our current aims either.

This paper presents an alternative approach to address the problem of the external decision-maker by combining the decision-making process design with an evolutionary game theoretic perspective. 
While  the former  captures the strategic behaviour of the decision-maker,  the latter can be used to formalise the evolutionary dynamics of the multiagent system and the strategic decisions within large populations exhibiting arbitrary population structures and social tensions.
In particular, we consider a multiagent system where the agents, \emph{distributed in a network}, interact  with their neighbours via the one-shot Prisoner's Dilemma (PD),  where uncooperative behaviour is preferred over cooperation \cite{Sigmund2001PNAS,santos2006pnas}.
As an outsider decision-maker, we aim to promote cooperation by interfering in the system,  rewarding particular agents in the population at specific moments; 
%In particular, at each time step, we can reward the agents with the cooperative behaviour. 
%However, as mentioned earlier, non-cooperation can reoccur over time, thus, the decision-maker has to repeatedly interfere in the system in order to maintain the desired ratio of cooperative agents over time.

The research question here is to identify when and how much to invest (i.e., pay the agents) at each time step, in order to achieve our desired ratio of cooperation within the system such that the total cost of interference is minimised.
%We formalise this problem of \emph{cost efficient sequential interference} as a bi-objective optimisation problem, where the first objective is to provide a sequential interference strategy (i.e., a sequence of interference decisions over time) that maximise the expected ratio of the cooperative agents within the population, while the second is to minimise the  total cost of interference.
We investigate two general classes or approaches of  interference strategies; the first is 
based on the current composition of the population while the second is based on local neighbourhood properties, in particular, for any agent being considered for investment we examine its current cooperativeness level (the number of its neighbours who will cooperate). 
These  two  classes represent a large fraction  of the sequential interference strategies in real--world scenarios,  requiring different levels of information in the decision making process.
While the first requires as input  the overall population  cooperativeness, the second requires more detailed, local information regarding  each neighbourhood to make a decision. They represent two different approaches of governing and incentivising  institutions: a large global institution overseeing the whole population  (such as the United Nations)  as opposed to multiple local institutions (such as regional or group-wide ones) \cite{vasconcelos2013bottom}.
%The last algorithms need to access the fitness levels of all players in the population. 
%For each class we consider when it is best to make an investment.
We are particularly interested in whether taking into account neighbourhood information will lead to more efficient interference and how this may be achieved.

The remainder of the paper is structured as follows: the next section provides a brief overview of the related work, this is followed by a detailed description of our model, its results and a final discussion. 
 
%This sequential decision-making problem, however, is typically difficult to solve (see Section~\ref{subsec:optimisation_model} for more details).
%Given this, we provide a sufficient condition of heuristics, where if a sequential interference strategy satisfies this condition, it can provide good performance (i.e., high population ratio of cooperative agents and low investment cost).

%In this paper, we systematically investigate how 
%We then investigate two natural strategy schemes, taken from real--world domains. %, that satisfy this condition.
%In particular,  the first strategy follows a scheme of fixed total investment per time step, where the investment is equally split among all the agents with the desired behaviour.
%In contrast, the second strategy rewards each agent, who ever follows the cooperative behaviour, with a fixed amount per time step.
%The reason we investigate these schemes is that together they represent a large fraction of the sequential interference strategies in real--world scenarios.
%In particular, the first scheme is motivated by interference strategies where the decision-maker has a fixed budget which is then refilled at each time step (e.g., annual financial budget of the WWF, or of other habitat management organisations). 
%On the other hand, the intuition of the second scheme is taken from real-world scenarios where the investments are based on individual merit, which are typically used in political or educational organisations (e.g., scholarships, or performance-based payments). 
%Given this, our contribution to the state of the art can be summarised as follows:
%\begin{itemize}
%\item We introduce the cost efficient sequential interference problem that is suitable for investigating how and when to invest into a closed evolutionary game system of multiple agents, in order to achieve some desired level of cooperation within the population.
%\item We introduce a new, bi-objective optimisation, model  to tackle this problem, for which we provide a sufficient condition of heuristics that guarantees high performance.  
%\item We investigate two natural interference strategies in more detail, and our findings provides novel insights on how to design efficient sequential interference strategies. In particular, we demonstrate that (i) across the different scenarios, an interference strategy must be thorough but not overdone; (ii) in many cases, the individual merit-based interference strategy leads to more efficient performance; and (iii) by spreading our support to sufficiently large groups of agents, the total expected cost of interference, which is needed to maintain a desired ratio of agents with good behaviour within the population, is decreased. 
%\end{itemize}

%\noindent
%The remainder of the paper is as follows.
%The next section reviews the existing related work.
%We then introduce our formal model in Section~\ref{section:model}.
%Section~\ref{section:optimisation} formalises the cost efficient interference problem.
%Section~\ref{section:evaluation} then describes the numerical evaluation results, and Section~\ref{section:conclusions} concludes.


==> IJCAI/related_work.tex <==
% !TEX root = ijcai18.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Related Work}
\label{section:related_work}

\noindent
In the literature of evolution of cooperation, different mechanisms of cooperation have been studied, including  direct and indirect reciprocity~\cite{nowak:2005:nature}, kin and group selections~\cite{traulsen:2006:pnas}, network reciprocity \cite{santos2006pnas}, punishment and rewarding~\cite{Sigmund2001PNAS}, and pre-commitments \cite{Han2017AAAI}. 
These mechanisms are incorporated as part of individual  strategic behaviours, in order to study how they  evolve and whether their evolution promotes a better outcome for cooperative behaviour.
These works, however, do not consider the influence of an exogenous decision-maker, but rather rely on the changes made by internal agents.
In contrast, our interference strategies are external, i.e. they are not incorporated into the individual strategy. In addition, the aim of our strategies is to minimise the cost of interference while guaranteeing  high levels of cooperation, contrary to past literature where the cost optimisation is often omitted. %~\footnote{How to interfere in a system where such internal mechanisms are already incorporated, e.g. in repeated games or when agents interact in a spatial network, are left for future work. However, we envisage that the cost of interference would be reduced as in such scenarios, agents have additional incentives to cooperate.}.
In this respect, our work is also different  from the modelling works of institutional incentives to  encourage  cooperation through costly  reward and punishment (see e.g., \cite{sigmund2010social,vasconcelos2013bottom}) as well as through enforcing agreements \cite{Han2017AAAI}. 

Closely related to the current work is the analysis in  \cite{han2015cost,han2014cost}  where cost-efficient interference is  studied in well-mixed populations (i.e. having a fully connected graph structure). Thus, the interference therein only depends on the composition of the population. In the more complex scenario of structured populations we consider in this paper, agents might have different types of neighbourhood. As shown below, taking into account neighbourhood properties leads to more cost-efficient interference strategies than that based solely on the population composition. 
		
Works on cooperation in social networks also assume that changes are initiated from inside the system~\cite{RaghunandanS12,SahraeiBBTW14,FranksGJ13,FranksGA14}.
Among them, more relevant to our paper is the recent work by Franks \emph{et al.}~\cite{FranksGJ13,FranksGA14}, which has explored the use of influencers on complex networks. However, these influencers are also part of the system and thus, similar to the cases mentioned above, this work does not consider external interference mechanisms. Given this, it does not address similar decision-making problems that we examine here. 
% 
Apart from these examples, some other works apply schemes of mechanism design to control the behaviour of the system.
Endriss \emph{et al.}~\cite{endriss2011incentive} %  ("incentive engineering for boolean games")
investigated how to tax games to incentivise certain behaviours in system equilibrium points and Wooldridge \emph{et al.}~\cite{Wooldridge12} % "bad equilibria and what to do about them" 
discussed the options to manipulate games in order to achieve desired behaviours. 
These works, however, assume that the decision-maker has full control on the agents within the systems, which allows her to both reward the good agents (i.e., those who follow the desired behaviours) and penalising the deviant ones. 
With our approach, the decision-maker has little or no control on the agents so they can rely only on rewarding schemes, nudging agents to adopt a given strategy. Moreover, mechanism design work typically does not focus on the cost of maintaining the desired behaviour, whereas cost optimisation is one of our objectives. 

Last but not least, Bachrach \emph{et al.}~\cite{Bachrach2009} % "the cost of stability"
investigated how much investment into a cooperative game is needed in order to ensure that a certain coalition structure is stable.
This work, however, only considers non-evolving systems with a single time step, and thus, interference can only be applied once.
In contrast, in our system, due to its evolutionary dynamics (and stochasticity), interference is repeatedly carried out over time (see the next section for more detail).
Thus, the related work (above) cannot be applied directly to our approach.




==> Promoting Fair Proposers, Fair Responders or Both_ Cost-Efficient Interference in the Spatial Ultimatum Game/IJCAI/Introduction.tex <==
% !TEX root = ijcai18.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}
\label{section:intro}
The problem of understanding and predicting  collective behaviours of agents in evolving multiagent systems is a well studied research topic in evolutionary game theory, as it can be found in a variety of real-world situations, ranging from ecosystems to human organisations and social networks~\cite{santos2006pnas,Sigmund2001PNAS,tuyls2007evolutionary,RaghunandanS12,HanJaamas2016,SahraeiBBTW14}. In this context, cooperation is typically assumed to emerge from the combined actions of participating agents within the system. 
%For example, in a country's political scene, cooperative behaviour is encouraged by its participating political parties, in order to achieve economical prosperity. 
%Similarly, in wildlife ecosystems, cooperation is assumed to be advocated by the members of the species in order to survive.
%
However, in many scenarios, such behaviours are advocated and promoted by an \emph{exogenous agent}, which  is not part of the system, calling for a new set of heuristics capable of {\it engineering} a desired collective behaviour in a self-organised multiagent system. 
%For example, consider an international political/economical organisation (e.g., the United Nations, or the European Union) that is not part of a certain country's political life (and thus, can be considered as an outsider from that country's political parties' perspective), decides to promote a certain preferred political behaviour. 
%To do so, the organisation can provide financial support to political parties that choose to follow the preferred politics. 
%However, for the organisation, this political investment comes with a (financial) cost in the form of monetary expenses. 
%Thus, from a decision-maker perspective, a key challenge for the organisation is to decide whether and how to \emph{interfere} (i.e., invest to achieve certain changes) in that country's political scene, such that the desired political situation is achieved, while the total cost of interference (i.e., investment cost) is minimised.
%
For instance, consider a wildlife management organisation (e.g., the WWF) that aims  to maintain a desired level of biodiversity in a particular region.
To do so, the organisation,  not being  part of the region's eco-system, has to decide whether to modify the current population of some species, and if so, then when, and in what degree to \emph{interfere} in the eco-system (i.e., to modify the composition and the biodiversity of the population)~\cite{levin2000multiple}.
Note that since more efficient population controlling typically implies more physical actions, which requires higher (monetary) expenses in both human resources and equipment, the organisation has to achieve a balance between efficient wildlife management and a low total investment cost. 
Moreover, due to the evolutionary dynamics of the eco-system (e.g., frequency and structure dependence \cite{santos2006pnas}), undesired behaviours can reoccur over time, for example when the interference was not sufficiently strong in the past. 
Given this, the decision-maker also has to take into account the fact that she will have to repeatedly interfere in the eco-system in order to sustain the level of biodiversity over time.
That is, she has to find an efficient sequential interference strategy that leads to her desired goals, while also minimising the total cost of interference.

Although the (sequential) decision-making literature provides a number of techniques to tackle similar problems where the goal is to provide a sequence of decisions that lead to optimal behaviour of the system (e.g., the desired level of biodiversity) while minimising the total cost of making such decisions~\cite{Madani2004,GuhaMunagala2007,Bachrach2009,Tran-Thanh2012,DingEtAl2013}, these approaches typically ignore the fact that the agents, with whom the decision-maker has to interact, also have their own strategic behaviours that together drive the (evolutionary) dynamics of the system. 
Given this, we argue that such solutions will not be able to exploit the system characteristics, and thus, will fail in providing efficient performance in achieving the desired system status (e.g., the status quo between the fighting opponents, or the desired diversity of population).
%
On the other hand, game theoretic literature, which deals with these strategic behaviours, typically focuses on the extremes of the problem. 
In particular, researchers either assume that the system is fully closed (i.e., there are no outsider decision-makers) or the decision-maker has full control over the behaviour of the agents.
Typical models for the former are classical (both non-cooperative and coalitional) game theoretical models~\cite{Bachrach2009,AzizBH10,AadithyaMJ11}. 
The latter includes models from mechanism design, where the decision-maker is the system designer, and can define some set of norms and penalties such that the agents are  incentivised not to deviate from the desired behaviour~\cite{endriss2011incentive,Wooldridge12,LevitEtAl2013,HarrensteinTW14}. 
Given this, these works are not suitable to meet our current aims either.

This paper presents an alternative approach to address the problem of the external decision-maker by combining the decision-making process design with an evolutionary game theoretic perspective. 
While  the former  captures the strategic behaviour of the decision-maker,  the latter can be used to formalise the evolutionary dynamics of the multiagent system and the strategic decisions within large populations exhibiting arbitrary population structures and social tensions.
In particular, we consider a multiagent system where the agents, \emph{distributed in a network}, interact  with their neighbours via the one-shot Prisoner's Dilemma (PD),  where uncooperative behaviour is preferred over cooperation \cite{Sigmund2001PNAS,santos2006pnas}.
As an outsider decision-maker, we aim to promote cooperation by interfering in the system,  rewarding particular agents in the population at specific moments; 
%In particular, at each time step, we can reward the agents with the cooperative behaviour. 
%However, as mentioned earlier, non-cooperation can reoccur over time, thus, the decision-maker has to repeatedly interfere in the system in order to maintain the desired ratio of cooperative agents over time.

The research question here is to identify when and how much to invest (i.e., pay the agents) at each time step, in order to achieve our desired ratio of cooperation within the system such that the total cost of interference is minimised.
%We formalise this problem of \emph{cost efficient sequential interference} as a bi-objective optimisation problem, where the first objective is to provide a sequential interference strategy (i.e., a sequence of interference decisions over time) that maximise the expected ratio of the cooperative agents within the population, while the second is to minimise the  total cost of interference.
We investigate two general classes or approaches of  interference strategies; the first is 
based on the current composition of the population while the second is based on local neighbourhood properties, in particular, for any agent being considered for investment we examine its current cooperativeness level (the number of its neighbours who will cooperate). 
These  two  classes represent a large fraction  of the sequential interference strategies in real--world scenarios,  requiring different levels of information in the decision making process.
While the first requires as input  the overall population  cooperativeness, the second requires more detailed, local information regarding  each neighbourhood to make a decision. They represent two different approaches of governing and incentivising  institutions: a large global institution overseeing the whole population  (such as the United Nations)  as opposed to multiple local institutions (such as regional or group-wide ones) \cite{vasconcelos2013bottom}.
%The last algorithms need to access the fitness levels of all players in the population. 
%For each class we consider when it is best to make an investment.
We are particularly interested in whether taking into account neighbourhood information will lead to more efficient interference and how this may be achieved.

The remainder of the paper is structured as follows: the next section provides a brief overview of the related work, this is followed by a detailed description of our model, its results and a final discussion. 
 
%This sequential decision-making problem, however, is typically difficult to solve (see Section~\ref{subsec:optimisation_model} for more details).
%Given this, we provide a sufficient condition of heuristics, where if a sequential interference strategy satisfies this condition, it can provide good performance (i.e., high population ratio of cooperative agents and low investment cost).

%In this paper, we systematically investigate how 
%We then investigate two natural strategy schemes, taken from real--world domains. %, that satisfy this condition.
%In particular,  the first strategy follows a scheme of fixed total investment per time step, where the investment is equally split among all the agents with the desired behaviour.
%In contrast, the second strategy rewards each agent, who ever follows the cooperative behaviour, with a fixed amount per time step.
%The reason we investigate these schemes is that together they represent a large fraction of the sequential interference strategies in real--world scenarios.
%In particular, the first scheme is motivated by interference strategies where the decision-maker has a fixed budget which is then refilled at each time step (e.g., annual financial budget of the WWF, or of other habitat management organisations). 
%On the other hand, the intuition of the second scheme is taken from real-world scenarios where the investments are based on individual merit, which are typically used in political or educational organisations (e.g., scholarships, or performance-based payments). 
%Given this, our contribution to the state of the art can be summarised as follows:
%\begin{itemize}
%\item We introduce the cost efficient sequential interference problem that is suitable for investigating how and when to invest into a closed evolutionary game system of multiple agents, in order to achieve some desired level of cooperation within the population.
%\item We introduce a new, bi-objective optimisation, model  to tackle this problem, for which we provide a sufficient condition of heuristics that guarantees high performance.  
%\item We investigate two natural interference strategies in more detail, and our findings provides novel insights on how to design efficient sequential interference strategies. In particular, we demonstrate that (i) across the different scenarios, an interference strategy must be thorough but not overdone; (ii) in many cases, the individual merit-based interference strategy leads to more efficient performance; and (iii) by spreading our support to sufficiently large groups of agents, the total expected cost of interference, which is needed to maintain a desired ratio of agents with good behaviour within the population, is decreased. 
%\end{itemize}

%\noindent
%The remainder of the paper is as follows.
%The next section reviews the existing related work.
%We then introduce our formal model in Section~\ref{section:model}.
%Section~\ref{section:optimisation} formalises the cost efficient interference problem.
%Section~\ref{section:evaluation} then describes the numerical evaluation results, and Section~\ref{section:conclusions} concludes.


==> Promoting Fair Proposers, Fair Responders or Both_ Cost-Efficient Interference in the Spatial Ultimatum Game/IJCAI/related_work.tex <==
% !TEX root = ijcai18.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Related Work}
\label{section:related_work}

\noindent
In the literature of evolution of cooperation, different mechanisms of cooperation have been studied, including  direct and indirect reciprocity~\cite{nowak:2005:nature}, kin and group selections~\cite{traulsen:2006:pnas}, network reciprocity \cite{santos2006pnas}, punishment and rewarding~\cite{Sigmund2001PNAS}, and pre-commitments \cite{Han2017AAAI}. 
These mechanisms are incorporated as part of individual  strategic behaviours, in order to study how they  evolve and whether their evolution promotes a better outcome for cooperative behaviour.
These works, however, do not consider the influence of an exogenous decision-maker, but rather rely on the changes made by internal agents.
In contrast, our interference strategies are external, i.e. they are not incorporated into the individual strategy. In addition, the aim of our strategies is to minimise the cost of interference while guaranteeing  high levels of cooperation, contrary to past literature where the cost optimisation is often omitted. %~\footnote{How to interfere in a system where such internal mechanisms are already incorporated, e.g. in repeated games or when agents interact in a spatial network, are left for future work. However, we envisage that the cost of interference would be reduced as in such scenarios, agents have additional incentives to cooperate.}.
In this respect, our work is also different  from the modelling works of institutional incentives to  encourage  cooperation through costly  reward and punishment (see e.g., \cite{sigmund2010social,vasconcelos2013bottom}) as well as through enforcing agreements \cite{Han2017AAAI}. 

Closely related to the current work is the analysis in  \cite{han2015cost,han2014cost}  where cost-efficient interference is  studied in well-mixed populations (i.e. having a fully connected graph structure). Thus, the interference therein only depends on the composition of the population. In the more complex scenario of structured populations we consider in this paper, agents might have different types of neighbourhood. As shown below, taking into account neighbourhood properties leads to more cost-efficient interference strategies than that based solely on the population composition. 
		
Works on cooperation in social networks also assume that changes are initiated from inside the system~\cite{RaghunandanS12,SahraeiBBTW14,FranksGJ13,FranksGA14}.
Among them, more relevant to our paper is the recent work by Franks \emph{et al.}~\cite{FranksGJ13,FranksGA14}, which has explored the use of influencers on complex networks. However, these influencers are also part of the system and thus, similar to the cases mentioned above, this work does not consider external interference mechanisms. Given this, it does not address similar decision-making problems that we examine here. 
% 
Apart from these examples, some other works apply schemes of mechanism design to control the behaviour of the system.
Endriss \emph{et al.}~\cite{endriss2011incentive} %  ("incentive engineering for boolean games")
investigated how to tax games to incentivise certain behaviours in system equilibrium points and Wooldridge \emph{et al.}~\cite{Wooldridge12} % "bad equilibria and what to do about them" 
discussed the options to manipulate games in order to achieve desired behaviours. 
These works, however, assume that the decision-maker has full control on the agents within the systems, which allows her to both reward the good agents (i.e., those who follow the desired behaviours) and penalising the deviant ones. 
With our approach, the decision-maker has little or no control on the agents so they can rely only on rewarding schemes, nudging agents to adopt a given strategy. Moreover, mechanism design work typically does not focus on the cost of maintaining the desired behaviour, whereas cost optimisation is one of our objectives. 

Last but not least, Bachrach \emph{et al.}~\cite{Bachrach2009} % "the cost of stability"
investigated how much investment into a cooperative game is needed in order to ensure that a certain coalition structure is stable.
This work, however, only considers non-evolving systems with a single time step, and thus, interference can only be applied once.
In contrast, in our system, due to its evolutionary dynamics (and stochasticity), interference is repeatedly carried out over time (see the next section for more detail).
Thus, the related work (above) cannot be applied directly to our approach.



